SoK: Untangling File-based Encryption on Mobile Devices

File-based encryption (FBE) schemes have been developed by software vendors to address security concerns related to data storage. While methods of encrypting data-at-rest may seem relatively straightforward, the main proponents of these technologies in mobile devices have nonetheless created seemingly different FBE solutions. As most of the underlying design decisions are described either at a high-level in whitepapers, or are accessible at a low-level by examining the corresponding source code (Android) or through reverse-engineering (iOS), comparisons between schemes and discussions on their relative strengths are scarce. In this paper, we propose a formal framework for the study of file-based encryption systems, focusing on two prominent implementations: the FBE scheme used in Android and Linux operating systems, as well as the FBE scheme used in iOS. Our proposed formal model and our detailed description of the existing algorithms are based on documentation of diverse nature, such as whitepapers, technical reports, presentations and blog posts, among others. Using our framework we validate the security of the existing key derivation chains, as well as the security of the overall designs, under widely-known security assumptions for symmetric ciphers, such as IND-CPA or INT-CTXT security, in the random-oracle model.

==> old_stuff.tex <==
\begin{algorithm}[t]
	\SetKwProg{function}{function}{}{}
	\KwIn{$\textit{f}sblock,k$}
	\KwOut{$eblock$}
	\BlankLine
		\jia{decryption algorithm missing}\\
	\function{$\mathsf{ENC}^{\hspace{-3pt}\begin{scriptsize}\begin{tabular}{l}cipher\\\end{tabular}\end{scriptsize}}(\textit{f}sblock,k)$}{
	    $\mathsf{iv} \xleftarrow{} \mathsf{GetIV}(\textit{f}sblock,k.mode)$\\
	    $eblock \xleftarrow{} CIPHER(\textit{f}sblock, k.\mathsf{val},\mathsf{iv})$\\
        \Return $eblock$
	}
	\add{change to\\
	\KwIn{$\textit{f}content,k$}
	\KwOut{$econtent$}
	\BlankLine
	\function{$ENC^{\fileciph}(fcontent, k)$}{
	 \For {$\textit{f}sblock \in \textit{f}node.content$}{
	 $\mathsf{iv} \xleftarrow{} \mathsf{GetIV}(\textit{f}sblock,k.mode)$\\
     $eblock \xleftarrow{} CIPHER(\textit{f}sblock, k.\mathsf{val},\mathsf{iv})$\\
     $econtent \xleftarrow{} econtent \| eblock$ \\
        }
	}
	}
	
	\caption{Encrypt (Android \& *NIX systems)}
	\label{alg:seckey}
\end{algorithm}











%EXT4 Related

\begin{comment}

The adversarial model for the EXT4 encryption excludes all attacks except the "single point-in-time permanent offline compromise of the block device". Furthermore, authenticated encryption modes are not supported due to difficulties related to ciphertext expansion and adversaries targeting data integrity are not dealt with \cite{EXT4-whitepaper}. \mihai{David, does this affect our Security Model?} 

In order to provide protection against offline attacks EXT4 encryption uses the following ciphers: $AES-128-ECB$ to perform key derivation, $AES-256-CTS-CBC$ to encrypt file and directory names, and $AES-256-XTS$ to encrypt the file contents. 

In Algoritm \ref{alg:encryptfbe} we present the pseudo-code for the EXT4 FBE as described in \cite{EXT4-whitepaper}.


\jia{need to store all the info in enode; otherwise cannot decrypt without fnode} \\
\mihai{well spotted. thanks. I have just revisited this and it seems that there is a new version of the protocol where AES-256-CTS-CBC(k,n_p) used to generate the key for fnode.name has been replaced with the stronger? HKDF-SHA512(k). np should no longer be needed.}\footnote{For v2 encryption policies, the KDF is HKDF-SHA512. The master key is passed as the “input keying material”, no salt is used, and a distinct “application-specific information string” is used for each distinct key to be derived. For example, when a per-file encryption key is derived, the application-specific information string is the file’s nonce prefixed with “fscrypt\\0” and a context byte. Different context bytes are used for other types of derived keys. https://www.kernel.org/doc/html/latest/filesystems/fscrypt.html} \\
\jia{If not using $n_c, n_p$, then need to model these ''application-specific information string''. It is the input to the pseudorandom function and needs to be distinct to guarantee all the derived keys are different.}
\jia{If not using $n_c, n_p$, then need to model these ''application-specific information string''. It is the input to the pseudorandom function and needs to be distinct to guarantee all the derived keys are different.}

\mihai{given that the ''application-specific information string'' serves the same purpose as the $n_{c/p}$, hopefully we can model it the same way. It is claimed that it is unique so we can model it as a random. We could also define a generic derivation function that can be instantiated with either AES-256-CTS-CBC or HKDF-SHA512, depending on the pol used, and receives k and $n_{p/c}$ as a parameter given that the two functions are identical from a sec proof point of view. does this make sense?}




\jia{Yes, can write $KDF(k, n_c)$ for a general key derivation function which is modeled as a pseudorandom function in the security model. Also write $ENC^{file\mbox{-}ciph}$ for the cipher used to encrypt file content, instead of AES-256-XTS.}


\todo{Include Adiantum encryption mode\footnote{https://eprint.iacr.org/2018/720.pdf} in addition to our current (AES-256-XTS, AES-256-CTS-CBC)}
\todo{Update to reflect pol V2 in ext4 (cur). refer to pol v1 (still supported)}

\medskip\noindent\textbf{Master key derivation.} EXT4 encryption does not use the master keys directly, instead, it uses individual keys for each $node.name$ and each $node.content$. These keys are derived from the master key using the AES-256-ECB cipher and a random 128bit nonce which is used as the key of the cipher. The nonce is stored in plaintext along the node, i.e. in our notation the nonce is stored inside $node.meta$. This method was chosen to reduce the size of the cryptographic metadata stored on disk. It is noted however by the authors that this requires the derived key to be "equally as hard to compromise" as the original master key \cite{EXT4-whitepaper}. We give the pseudo-code for the key derivation in Algorithm \ref{alg:encryptfbe} lines 4-8 and 12-16.

\medskip\noindent\textbf{Protecting file names.} Like most filesystems EXT4 is structured in a tree-like format. This enables specific filesystem functionality, such as managing permissions, browsing contents, searching, deleting, etc., to be very efficient. The FBE enhancement to EXT4 has been implemented such that encrypted EXT4 filesystems will continue to have all the functionality of non-encrypted EXT4 filesystems.

As such, to support some of these operations, node names need to be encrypted using keys associated to the parent node, e.g. the name of a file is encrypted with the key corresponding to the directory where is it stored. This key is in turn derived from the master key associated to the parent node as described above. The AES-256-CTS-CBC cipher is used for encrypting node names as shown in Algorithm \ref{alg:encryptfbe} line 10. A constant $\mathsf{iv}$ value is used to be able to maintain equality relationship between encrypted and non-encrypted node names inside a specific parent node. Given that symmetric encryption is used the  decryption is similar to the encryption (Algorithm \ref{alg:decryptfbe}).


\medskip\noindent\textbf{Protecting the file content.} Node contents encryption is done on a per filesystem block basis. Each block has an initialisation vector, $\mathsf{iv}$, corresponding to the \textit{logical block offset within the file} \cite{EXT4-whitepaper}. In addition to the $\mathsf{iv}$ each node uses a unique node contents encryption key derived from a master key as described above. EXT4 encryption uses the AES-256-XTS cipher to perform this node contents encryption and decryption. The details of this operation are presented in Algorithm \ref{alg:encryptfbe} lines 11-18 and Algorithm \ref{alg:decryptfbe} lines 8-10, respectively.



\end{comment}


%old ext4 algo

\begin{comment}
\begin{algorithm}[t]
	\SetKwProg{function}{function}{}{}
	\KwIn{$\textit{f}node,kid$}
	\KwOut{$enode$}
	\BlankLine
	\function{$\mathsf{\Encrypt}(\textit{f}node,kid)$}{
		$k  \xleftarrow{} {} GetKeyFromKernelKeyring(kid)$\\
		$\enode.parent = \fnode.parent$ \\
		\If {$k$}{
		    \tcc{1. Node name}
		    $n_{p} \xleftarrow{} \enode.parent.meta$\\
		    \If {$n_{p} = null$}{
                \tcc{Encrypting for the first time.}
                $n_{p} \xleftarrow{R} \{0,1\}^{128}$\\
               $\enode.parent.meta \xleftarrow{} n_{p}$\\
            }
            \BlankLine
            \tcc{Derive node name key and encrypt}
            $k_{n} \xleftarrow{} MasterKDF(k, n_{p})$\\
            $\mathsf{iv} \xleftarrow{} \{0\}^{256}$\\
            \vspace{-6pt}
            $enode.name \xleftarrow{} ENC^{\hspace{-3pt}\begin{scriptsize}\begin{tabular}{l}metadata-\\cipher\\\end{tabular}\end{scriptsize}}(\textit{f}node.name, k_{n}, \mathsf{iv})$
            
            \BlankLine
            \BlankLine
            \BlankLine
            
            \tcc{2. Node contents}
            \If {$\textit{f}node = file$}{
                $n_{c} \xleftarrow{} \textit{f}node.meta$\\
    		    \If {$n_{c} = null$}{
                    $n_{c} \xleftarrow{R} \{0,1\}^{128}$\\
                   $\enode.meta \xleftarrow{} n_{c}$\\
                }
                \BlankLine
                \tcc{Derive file content key and encrypt}
                $k_{c} \xleftarrow{} MasterKDF(k, n_{c})$\\
                $enode.content \xleftarrow{} ENC^{\hspace{-3pt}\begin{scriptsize}\begin{tabular}{l}data-\\cipher\\\end{tabular}\end{scriptsize}}(\textit{f}node.content, k_{c})$
            }
            \Return $enode$
		} \Else {
            \Return $\bot$
		}
	}
	\caption{File encryption in EXT4 filesystems (Android \& *NIX systems)}
	\label{alg:encryptfbe}
\end{algorithm}

\begin{algorithm}[t]
	\SetKwProg{function}{function}{}{}
	\KwIn{$enode,kid$}
	\KwOut{$\textit{f}node$}
		
	\BlankLine
	\function{$\mathsf{\Decrypt}(enode,kid)$}{
		$k  \xleftarrow{} {} GetKeyFromKernelKeyring(kid)$\\
	$\fnode.parent = \enode.parent$ \\
		\If {$k$}{
		    \tcc{1. Node name}
		    $n_{p} \xleftarrow{} \textit{f}node.parent.meta$\\
            \BlankLine
            \tcc{Derive node name key and encrypt}
            $k_{n} \xleftarrow{} MasterKDF(k, n_{p})$\\
            $\mathsf{iv} \xleftarrow{} \{0\}^{256}$\\
            \vspace{-6pt}
            $\textit{f}node.name \xleftarrow{} DEC^{\hspace{-3pt}\begin{scriptsize}\begin{tabular}{l}metadata\\cipher\\\end{tabular}\end{scriptsize}}(enode.name, k_{n}, \mathsf{iv})$
            
            \BlankLine
            \BlankLine
            \BlankLine
            
            \tcc{2. Node contents}
            \If {$\enode = file$}{
                \BlankLine
                \tcc{Derive file content key and encrypt}
                $n_{c} \xleftarrow{} \enode.meta$\\
                 $k_{c} \xleftarrow{} MasterKDF(k, n_{c})$\\
                $\textit{f}node.content \xleftarrow{} DEC^{\hspace{-3pt}\begin{scriptsize}\begin{tabular}{l}data-\\cipher\\\end{tabular}\end{scriptsize}}(enode.content, k_{c})$ \\
                $\fnode.meta = n_c$ \\
            }
            \Return $\textit{f}node$
		} \Else {
            \Return $\bot$
		}
	}
	\caption{File decryption in EXT4 filesystems (Android \& *NIX systems)}
	\label{alg:decryptfbe}
\end{algorithm}

\end{comment}














%IOS related

\begin{comment}
\begin{algorithm}[h]
	\SetKwProg{function}{function}{}{}
	\KwIn{$\lambda,path,pol$}
    \ExecCon{Userland}
	\BlankLine
	\function{$BUILD\_KEY(\lambda, path, pol)$}{
        \uIf{pol = Complete}{
        }\uElseIf{pol = CompleteUnlessOpen} {
        }\uElseIf{pol = CompleteUntilFirstUserAuthentication} {
        }\uElseIf{pol = None} {
        }
        \Return $k_{enc\_master}$
    }
	\caption{iOS BuildKey}
	\label{alg:iosbuildkey}
\end{algorithm}

\begin{algorithm}[h]
	\SetKwProg{function}{function}{}{}
	\KwIn{$k_{em},pol$}
	\KwOut{$kid$}
    \Constants{$k_{uid},ciph\_hw$}
    \ExecCon{SE}
	\BlankLine
   \function{$ProvisionKey(k_{em}, pol)$}{
       $k_{m} \xleftarrow{} null$\\
        \uIf{$pol = Complete$}{
            $k_p \xleftarrow{} pol.GET_PDF()$\\
            $SE\_COMPLETE\_PROVISION(k_p)$\\
        }\uElseIf{$pol = CompleteUnlessOpen$} {
        }\uElseIf{$pol = CompleteUntilFirstUserAuthentication$} {
        }\uElseIf{$pol = None$} {
            $k_{wkek} \xleftarrow{} pol.k_{wkek}$\\
            $ciph \xleftarrow{} pol.cipher$\\
            $k_{kek} \xleftarrow{} DEC^{ciph\_hw}(k_{uid}, k_{wkek})$\\
            $k_{m} \xleftarrow{} DEC^{ciph}(k_{kek}, k_{em})$\\
        }
        \If{$k_{m} \neq null$} {
            $kid \xleftarrow{} Install(k_{m})$\\
            \Return $kid$
        }
    }
    \BlankLine
    \nonl\hrulefill
    \BlankLine
	\KwIn{$k_p$}
    \ExecCon{Secure Enclave}
	\BlankLine
    \setcounter{AlgoLine}{0}
    \function{$SE\_COMPLETE\_PROVISION(k_p)$}{
        $k_{enc\_p} \xleftarrow{} ENC(k_{uid}, k_p)$\\
        \tcc{The following KDF is iterated to achieve time-delay}
        $k_w \xleftarrow{} KDF(k_{enc\_p})$
    }
	\caption{iOS ProvisionKey}
	\label{alg:iosprovisionkey}
\end{algorithm}
\end{comment}

% END OF COMMENTED OUT (OLD) WORK! WHICH STARTED ABOVE

\begin{comment}
\subsection{iOS Case Study}

Although we are not able to provide a formal description of file encryption in iOS, we can provide some high level details. 

\medskip\noindent\textbf{File encryption.} 
For file encryption, iOS uses AES-128-XTS. The IV for each encryption is calculated as the block offset into the file, encrypted with the SHA1 hash of the master key $k_c$.

\medskip\noindent\textbf{Dedicated Storage Controller} 
Of most notable difference to Android's implementation, is the offloading and physical separation of encryption operations to a dedicated storage controller (DSC). Crucially, this affords the benefit of never exposing a per-file encryption key to the application processor (AP). To achieve this, the per-file key $k_c$ is communicated to the DSC over a secure channel. This channel is set up at boot time through negotiation of an ephemeral key $k_{eph}$ between the SEP and DSC \chris{is there any info on how this is generated/negotiated? Perhaps in that defcon/blackhat ios RE talk?}. Hereinafter, file encryption/decryption requests, made to the SEP, result in a wrapped file key corresponding to $ENC^{ciph}(k_{eph},k_{c})$ transported to the DSC via the kernel \cite{krsticios}. The DSC is then able to unwrap this value and encrypt/decrypt the file. 
\end{comment}




